A Faster Deterministic Algorithm for Mader's $\mathcal{S}$-Path Packing

Given an undirected graph $G = (V,E)$ with a set of terminals $T\subseteq V$ partitioned into a family $\mathcal{S}$ of disjoint blocks, find the maximum number of vertex-disjoint paths whose endpoints belong to two distinct blocks while no other internal vertex is a terminal. This problem is called Mader's $\mathcal{S}$-path packing. It has been of remarkable interest as a common generalization of the non-bipartite matching and vertex-disjoint $s\text{-}t$ paths problem. This paper presents a new deterministic algorithm for this problem via known reduction to linear matroid parity. The algorithm utilizes the augmenting-path algorithm of Gabow and Stallmann (1986), while replacing costly matrix operations between augmentation steps with a faster algorithm that exploits the original $\mathcal{S}$-path packing instance. The proposed algorithm runs in $O(mnk)$ time, where $n = |V|$, $m = |E|$, and $k = |T|\le n$. This improves on the previous best bound $O(mn^{\omega})$ for deterministic algorithms, where $\omega\ge2$ denotes the matrix multiplication exponent.

==> discussion.tex <==
\section{Discussion}

We expect that our techniques desirably contributes to devising efficient solutions for other generalization of Mader's problem that allow for similar reduction to (weighted) linear matroid parity e.g.,~\cite{tanigawa2016packing,yamaguchi2016packing,yamaguchi2016shortest}.

The present approach would not immediately imply as efficient a combinatorial algorithm as \autoref{thm:main}, unless we identify any combinatorial companion for arithmetic operations involved inside the augmenting-path algorithm~\cite{gabow1986augmenting}.

Lastly, it would be a promising direction to seek a ``dual'' partition for Mader's min-max theorem~\cite{mader1978die,lovasz1980matroid}, which certifies that the obtained $\cS$-path packing is the maximum.
A potential key may lie in the dual solution for Lov{\'a}sz's min-max theorem~\cite{lovasz1980selecting} that can be constructed when the augmenting-path algorithm terminates.\footnote{Gabow and Stallmann~\cite{gabow1986augmenting} indeed prove the maximality of a solution by establishing \autoref{prop:dual}.}
Note nevertheless that it is not straightforward to interpret this dual solution in the context of Mader's problem, partly because some vectors in $A$ can be neither singletons nor vertex-/edge-twins.

\begin{proposition}[\cite{gabow1986augmenting}]\thlabel{prop:dual}
  A partition $(L_1,\ldots,L_p)$ of $L$ is said to be a parity partition if and only if every line is contained in some $L_i$.
  When the augmenting-path algorithm halts without augmentation, one can obtain an independent set of vectors $A$ and a parity partition $(L_1,\ldots,L_p)$ that satisfies
  \begin{align}
    |E[B]| = |A| + \sum_{i=1}^{p} \left\lfloor\frac{\rank(L_i\cup A) - |A|}{2}\right\rfloor.
  \end{align}
\end{proposition}

\begin{theorem}[\cite{mader1978die,lovasz1980matroid}\footnote{Another equivalent formulation about this duality is also notable~\cite{sebHo2004path}.}]
  The maximum size of a $\cS$-path packing is equal to
  \begin{align}
    \min_{V_0,V_1,\ldots,V_p} |V_0| + \sum_{i=1}^p \left\lfloor\frac{|V_i|}{2}\right\rfloor,
  \end{align}
  where $(V_0,V_1,\ldots,V_p)$ runs over all partitions of $V$ such that any $\cS$-path passes $V_0$ or $E[V_i]$, and defines
  \begin{align}
    B_i &\coloneqq (V_i\cap T) \cup \{v\in V_i \mid \exists v'\in V\setminus(V_0\cup V_i),\ \{v, v'\}\in E \}
    &\forall i\in\{1,\ldots,p\}.
  \end{align}
\end{theorem}
